Chemically consistent evolution of galaxies: galaxy models compared to DLA systems

We have extended our chemical and cosmological galaxy evolution model to calculate the abundance evolution for altogether 16 different elements in spiral galaxies in a chemically consistent way which is a considerable step towards a more realistic galaxy modeling. Our models well reproduce observed average HII region abundances in all spiral types. All observed element abundances in DLA systems have been compiled. The conformity between observed and calculated abundances over the redshift range from z=4.5 through z=0.4 indicates that DLA galaxies may well evolve into the full range of present- day spiral galaxies from Sa through Sd. Comparison of our chemically consistent models with models using only solar metallicity input physics shows that differences in the redshift evolution are small for some elements but large for others. For those elements with large differences the chemically consistent models provide significant better agreement with observed DLA abundances. For typical spiral galaxies the star formation histories of our models clearly bridge the gap between high redshift DLA systems and the nearby spiral galaxy population. The slow redshift evolution of DLA abundances is understood in terms of the long star formation timescales in galactic and proto-galactic disks. Towards lower redshift z < 1.5 our models indicate that early type spirals drop out of the DLA samples as their gas content falls below ~50%. Implications for optical identification are discussed.

==> SNII_data/Z=0Zsun_tex <==
 12&~~  6.39&~~  4.08&~~  .043&~~  .000&~~  .067&~~  .004&~~  .000&~~  .025&~~  .009&~~  .002&~~  .001&~~  .081&~~  .009&~~  .0006&~~  .0007&~~  .0002&~~ 10.72&~~  .07 \cr
 13&~~  6.83&~~  4.42&~~  .068&~~  .000&~~  .137&~~  .015&~~  .001&~~  .034&~~  .014&~~  .003&~~  .003&~~  .191&~~  .035&~~  .0029&~~  .0013&~~  .0006&~~ 11.79&~~  .29 \cr
 15&~~  7.69&~~  4.90&~~  .145&~~  .000&~~  .400&~~  .034&~~  .001&~~  .069&~~  .026&~~  .005&~~  .004&~~  .161&~~  .014&~~  .0007&~~  .0011&~~  .0006&~~ 13.55&~~  .73 \cr
 18&~~  8.85&~~  5.70&~~  .110&~~  .000&~~  .030&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 14.69&~~  .00 \cr
 20&~~  9.56&~~  6.32&~~  .090&~~  .000&~~  .009&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 15.98&~~  .01 \cr
 22&~~ 10.20&~~  7.10&~~  .277&~~  .000&~~ 1.850&~~  .095&~~  .002&~~  .166&~~  .110&~~  .025&~~  .024&~~  .169&~~  .011&~~  .0007&~~  .0027&~~  .0008&~~ 20.60&~~ 2.75 \cr
 25&~~ 11.40&~~  7.33&~~  .083&~~  .000&~~  .010&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 18.82&~~ -.02 \cr
 30&~~ 12.80&~~  9.11&~~  .109&~~  .004&~~  .027&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 22.05&~~  .00 \cr
 30\s&~~ 12.80&~~  9.30&~~  .348&~~  .004&~~ 4.350&~~  .249&~~  .006&~~  .124&~~  .046&~~  .009&~~  .009&~~  .325&~~  .041&~~  .0031&~~  .0036&~~  .0008&~~ 28.67&~~ 3.67 \cr
 35&~~ 14.20&~~  8.17&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 22.37&~~  .00 \cr
 35\s&~~ 14.30&~~ 10.60&~~  .349&~~  .000&~~ 1.920&~~  .048&~~  .001&~~  .002&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 27.60&~~ 1.38 \cr
 35\ds&~~ 14.30&~~ 10.70&~~  .404&~~  .000&~~ 5.580&~~  .239&~~  .005&~~  .211&~~  .090&~~  .018&~~  .018&~~  .578&~~  .032&~~  .0011&~~  .0060&~~  .0014&~~ 33.42&~~ 3.70 \cr
 40&~~ 15.00&~~  8.63&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 23.63&~~  .00 \cr
 40\s&~~ 15.20&~~ 12.00&~~  .285&~~  .000&~~  .578&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 28.07&~~  .02 \cr
 40\ds&~~ 15.20&~~ 12.00&~~  .482&~~  .000&~~ 7.260&~~  .281&~~  .006&~~  .344&~~  .163&~~  .033&~~  .031&~~  .725&~~  .041&~~  .0025&~~  .0085&~~  .0018&~~ 38.17&~~ 4.17 \cr

==> SNII_data/Z=10-4Zsun_tex <==
 12&~~  6.39&~~  3.91&~~  .074&~~  .000&~~  .146&~~  .009&~~  .000&~~  .060&~~  .048&~~  .012&~~  .012&~~  .055&~~  .003&~~  .0004&~~  .0010&~~  .0002&~~ 10.78&~~  .56 \cr
 13&~~  6.82&~~  4.31&~~  .109&~~  .000&~~  .181&~~  .008&~~  .000&~~  .052&~~  .028&~~  .006&~~  .005&~~  .090&~~  .004&~~  .0004&~~  .0016&~~  .0003&~~ 11.63&~~  .14 \cr
 15&~~  7.64&~~  5.08&~~  .143&~~  .000&~~  .383&~~  .018&~~  .001&~~  .053&~~  .024&~~  .005&~~  .004&~~  .064&~~  .003&~~  .0003&~~  .0013&~~  .0002&~~ 13.45&~~  .24 \cr
 18&~~  8.80&~~  6.12&~~  .219&~~  .000&~~  .766&~~  .058&~~  .002&~~  .098&~~  .038&~~  .007&~~  .006&~~  .162&~~  .008&~~  .0008&~~  .0019&~~  .0006&~~ 16.50&~~ 1.29 \cr
 20&~~  9.22&~~  6.58&~~  .215&~~  .000&~~ 1.510&~~  .017&~~  .001&~~  .242&~~  .143&~~  .034&~~  .019&~~  .091&~~  .001&~~  .0000&~~  .0039&~~  .0006&~~ 18.14&~~  .34 \cr
 22&~~  9.95&~~  7.42&~~  .273&~~  .000&~~ 1.730&~~  .033&~~  .001&~~  .280&~~  .167&~~  .036&~~  .023&~~  .124&~~  .003&~~  .0001&~~  .0040&~~  .0006&~~ 20.11&~~  .32 \cr
 25&~~ 10.70&~~  8.53&~~  .295&~~  .000&~~ 2.780&~~  .096&~~  .004&~~  .362&~~  .164&~~  .031&~~  .019&~~  .204&~~  .011&~~  .0004&~~  .0033&~~  .0008&~~ 23.29&~~  .38 \cr
 30&~~ 12.00&~~ 10.10&~~  .333&~~  .000&~~ 4.070&~~  .254&~~  .008&~~  .098&~~  .003&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 27.33&~~ 1.70 \cr
 30\s&~~ 12.00&~~ 10.10&~~  .333&~~  .000&~~ 4.340&~~  .264&~~  .008&~~  .264&~~  .089&~~  .018&~~  .016&~~  .210&~~  .008&~~  .0003&~~  .0034&~~  .0006&~~ 28.11&~~ 1.62 \cr
 35\s&~~ 13.20&~~ 11.80&~~  .358&~~  .000&~~ 5.550&~~  .330&~~  .009&~~  .097&~~  .003&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 32.18&~~ 2.59 \cr
 35\ds&~~ 13.20&~~ 11.90&~~  .358&~~  .000&~~ 5.620&~~  .328&~~  .009&~~  .272&~~  .112&~~  .023&~~  .022&~~  .583&~~  .031&~~  .0014&~~  .0067&~~  .0014&~~ 33.30&~~ 2.50 \cr
 35&~~ 13.20&~~ 11.70&~~  .164&~~  .000&~~  .026&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 25.09&~~  .00 \cr
 40&~~ 14.30&~~ 12.10&~~  .080&~~  .000&~~  .007&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 26.49&~~  .01 \cr
 40\s&~~ 14.30&~~ 13.60&~~  .420&~~  .000&~~ 6.200&~~  .284&~~  .007&~~  .036&~~  .001&~~  .000&~~  .000&~~  .000&~~  .000&~~  .0000&~~  .0000&~~  .0000&~~ 36.11&~~ 3.49 \cr
 40\ds&~~ 14.30&~~ 13.60&~~  .420&~~  .000&~~ 6.850&~~  .322&~~  .008&~~  .370&~~  .176&~~  .036&~~  .034&~~  .692&~~  .043&~~  .0019&~~  .0097&~~  .0023&~~ 38.12&~~ 3.29 \cr


==> SNII_data/Z=Zsun_tex <==
%\noalign {\smallskip Z = ~\Zsun}
 12&~~  5.96&~~  4.11&~~  .082&~~  .036&~~  .219&~~  .011&~~  .001&~~  .093&~~  .079&~~  .027&~~  .015&~~  .059&~~  .010&~~  .0012&~~  .0010&~~  .0005&~~ 10.74&  .33 \cr
 13&~~  6.32&~~  4.51&~~  .115&~~  .047&~~  .275&~~  .023&~~  .002&~~  .062&~~  .028&~~  .005&~~  .004&~~  .151&~~  .018&~~  .0023&~~  .0014&~~  .0007&~~ 11.62&  .49 \cr
 15&~~  6.98&~~  5.24&~~  .162&~~  .054&~~  .685&~~  .040&~~  .005&~~  .116&~~  .066&~~  .015&~~  .011&~~  .138&~~  .012&~~  .0014&~~  .0021&~~  .0011&~~ 13.65&  .90 \cr
 18&~~  7.89&~~  6.28&~~  .249&~~  .057&~~ 1.146&~~  .077&~~  .010&~~  .146&~~  .059&~~  .010&~~  .007&~~  .093&~~  .006&~~  .0005&~~  .0023&~~  .0012&~~ 16.34& 1.87 \cr
 20&~~  8.24&~~  6.72&~~  .214&~~  .060&~~ 1.953&~~  .049&~~  .004&~~  .300&~~  .176&~~  .037&~~  .015&~~  .120&~~  .008&~~  .0008&~~  .0036&~~  .0017&~~ 18.04&  .76 \cr
 22&~~  8.79&~~  7.51&~~  .242&~~  .067&~~ 2.385&~~  .062&~~  .008&~~  .382&~~  .190&~~  .036&~~  .018&~~  .241&~~  .019&~~  .0019&~~  .0044&~~  .0021&~~ 20.09&  .64 \cr
 25&~~  9.40&~~  8.64&~~  .324&~~  .080&~~ 3.254&~~  .162&~~  .025&~~  .339&~~  .149&~~  .027&~~  .017&~~  .169&~~  .013&~~  .0015&~~  .0031&~~  .0031&~~ 23.07& 2.01 \cr
 30&~~ 10.50&~~ 10.40&~~  .288&~~  .104&~~ 3.652&~~  .270&~~  .040&~~  .141&~~  .016&~~  .002&~~  .001&~~  .029&~~  .004&~~  .0015&~~  .0004&~~  .0003&~~ 25.90& 1.74 \cr
30\s&~~ 10.50&~~ 10.40&~~  .292&~~  .104&~~ 4.882&~~  .346&~~  .051&~~  .384&~~  .108&~~  .019&~~  .013&~~  .481&~~  .053&~~  .0042&~~  .0047&~~  .0026&~~ 28.16& 1.83 \cr
 35&~~ 11.50&~~ 11.90&~~  .303&~~  .125&~~ 3.072&~~  .188&~~  .030&~~  .059&~~  .012&~~  .002&~~  .002&~~  .032&~~  .004&~~  .0013&~~  .0005&~~  .0004&~~ 27.82& 2.12 \cr
35\s&~~ 11.50&~~ 11.90&~~  .322&~~  .125&~~ 5.822&~~  .392&~~  .064&~~  .166&~~  .019&~~  .003&~~  .002&~~  .032&~~  .006&~~  .0026&~~  .0005&~~  .0004&~~ 31.33& 3.11 \cr
35\ds&~~ 11.50&~~ 12.00&~~  .322&~~  .125&~~ 6.362&~~  .407&~~  .066&~~  .494&~~  .179&~~  .032&~~  .024&~~  .625&~~  .076&~~  .0059&~~  .0062&~~  .0060&~~ 33.23& 3.01 \cr
 40&~~ 11.10&~~ 13.00&~~  .315&~~  .141&~~ 2.361&~~  .124&~~  .021&~~  .031&~~  .011&~~  .002&~~  .002&~~  .032&~~  .003&~~  .0010&~~  .0005&~~  .0004&~~ 27.67& 1.90 \cr
40\s&~~ 11.10&~~ 13.00&~~  .365&~~  .141&~~ 6.031&~~  .363&~~  .065&~~  .080&~~  .013&~~  .003&~~  .002&~~  .033&~~  .006&~~  .0027&~~  .0005&~~  .0004&~~ 32.55& 4.13 \cr
40\ds&~~ 11.10&~~ 13.00&~~  .370&~~  .141&~~ 7.631&~~  .449&~~  .077&~~  .621&~~  .248&~~  .043&~~  .032&~~  .760&~~  .077&~~  .0076&~~  .0100&~~  .0051&~~ 35.98& 3.91 \cr

